Answering Private Linear Queries Adaptively using the Common Mechanism

When analyzing confidential data through a privacy filter, a data scientist often needs to decide which queries will best support their intended analysis. For example, an analyst may wish to study noisy two-way marginals in a dataset produced by a mechanism M1. But, if the data are relatively sparse, the analyst may choose to examine noisy one-way marginals, produced by a mechanism M2 instead. Since the choice of whether to use M1 or M2 is data-dependent, a typical differentially private workflow is to first split the privacy loss budget rho into two parts: rho1 and rho2, then use the first part rho1 to determine which mechanism to use, and the remainder rho2 to obtain noisy answers from the chosen mechanism. In a sense, the first step seems wasteful because it takes away part of the privacy loss budget that could have been used to make the query answers more accurate. In this paper, we consider the question of whether the choice between M1 and M2 can be performed without wasting any privacy loss budget. For linear queries, we propose a method for decomposing M1 and M2 into three parts: (1) a mechanism M* that captures their shared information, (2) a mechanism M1' that captures information that is specific to M1, (3) a mechanism M2' that captures information that is specific to M2. Running M* and M1' together is completely equivalent to running M1 (both in terms of query answer accuracy and total privacy cost rho). Similarly, running M* and M2' together is completely equivalent to running M2. Since M* will be used no matter what, the analyst can use its output to decide whether to subsequently run M1'(thus recreating the analysis supported by M1) or M2'(recreating the analysis supported by M2), without wasting privacy loss budget.

==> algorithm.tex <==









==> extra.tex <==

\subsection{Shared Information}
We hope that the common queries chosen contain shared information of the given mechanisms. In other word, the answer to the common queries can be derived by linear combinations of the original mechanism, with additional noise independent to the original queries. We define one mechanism is answerable from another mechanism as follows,

It means that $\comb=A_i \bmat_i$ and $\comvar = A_i \covar_i A_i^T + \sigma_i^2 C_i C_i^T$. For simplicity we denote $\mech_1(\data) = \mech_2(\data)$ when the distribution of $\mech_1(\data)$ is the same as the distribution of $\mech_2(\data)$.

Let's look at the mechanisms $\mech_1, \mech_2, \commech$ in the example \ref{example:sumquery}, because $\commech(\data) = \mech_1 (\data) + \sqrt{3} N(0, \sigma^2)$, we say $\commech$ is answerable from $\mech_1$. Similarly, because $\commech (\data)= A_2 \mech_2 (\data)$, where $A_2 = [ 1 ~ 1 ~ 1 ~ 1 ]$, we say $\commech$ is answerable from $\mech_2$. Note that $\commech$ is answerable from $\mech_1$ and $\mech_2$, hence we can say $\commech$ shares information between $\mech_1$ and $\mech_2$, which leads to the following definition,

\begin{definition}
We say that $\commech$ is a common candidate to $\mech_i$ and $\mech_j$ if $\commech$ is answerable from $\mech_i$ and answerable from $\mech_j$
\end{definition}

It requires extra effort to compute the coefficients $A_i, C_i$ in definition \ref{def:answer}, which is inconvenient for validation. There is an equivalent way to check whether one mechanism is answerable from the other or not, which is less intuitive but easier for validation. The following theorem gives necessary and sufficient conditions about when $\mech_1$ is answerable from $\mech_2$.


Here the generalized inequality $\preceq$ means that matrices are comparing in the Loewner order \cite{horn2012matrix}, for two matrices $X, Y$,  $X \preceq Y$ means that $Y-X$ is a positive semi-definite matrix. From theorem \ref{thm:answer} we see that the term $\bmat^T (\covar)^{-1} \bmat$ plays an important role in determining whether one mechanism is answerable from the other. Recall that the privacy cost of $\mech$ is $\Delta_M = \max_{i} \sqrt{ \left( \bmat^T \covar^{-1} B \right) [i][i]}$. If $\mech_1$ is answerable from $\mech_2$, then the privacy cost $\Delta_{\mech_1} \leq \Delta_{\mech_2}$. Due to the connection between privacy cost, we define $\bmat^T (\covar)^{-1} \bmat$ as the privacy cost matrix of $\mech$.

\begin{definition}
\label{def:pcostmat}
Given a mechanism $\mech(\data) = \bmat \data + N(\vec{0}, \covar)$, the privacy cost matrix of $\mech$ is defined as $\Phi_{\mech} = \bmat^T \covar^{-1} B$.
\end{definition}

In example \ref{example:sumquery}, $\Phi_{\commech} = \frac{1}{4\sigma^2} \vec{1}^T \vec{1}$, $\Phi_{\mech_1} = \frac{1}{\sigma^2} \vec{1}^T \vec{1}$, here $\vec{1} = [1~1~1~1]$ is the sum query. $\Phi_{\mech_2} = \frac{1}{\sigma^2} \mat{I}$, here $\mat{I} \in \mathbb{R}^{4\times 4}$ is the identity query. Because $\Phi_{\commech} \preceq \Phi_{\mech_1}$, $\Phi_{\commech} \preceq \Phi_{\mech_2}$, we can say $\commech$ is a common candidate to $\mech_1$ and $\mech_2$.

Privacy cost matrices can not only be used to validate common candidates, but also be used to find alternative ways to answer a given mechanism. Suppose the privacy cost matrices of two mechanisms are the same, $\Phi_{\mech_1} = \Phi_{\mech_2}$ and we want to estimate the dataset using $\mech_1$ by solving the following problem,

\begin{align*}
    \hat{\data} = \argmin_{\vec{z} \geq 0} \left( \mnorm{ \bmat \vec{z} - \mech (\data) } + \lambda \| \vec{z}\|_2 \right)
\end{align*}

Instead of answering $\mech_1(\data)$ directly, we can answer $\mech_2(\data)$ first, and then construct $\mech_1(\data)$ based on $\mech_2(\data)$ because $\mech_1(\data)$ is answerable from $\mech_2(\data)$. In this case, answering $\mech_1$ is equivalent to answering $\mech_2$, which leads to the following definition,  

\begin{definition}
We say that $\mech_1(\data) = \bmat_1 \data + N(0, \covar_1)$ is equivalent to $\mech_2(\data) = \bmat_2 \data + N(0, \covar_2)$, if $\Phi_{\mech_1} = \Phi_{\mech_2}$. That is, the privacy cost matrix of $\mech_1$ and $\mech_2$ are the same.
\end{definition}


We find it helpful to analyze mechanisms that have a linearly row independent query matrix and an identity covariance matrix. Given a mechanism, we can always find an equivalent mechanism that holds the above mentioned properties.

------------

Note that it doesn't matter which mechanism we choose to answer, as long as they are equivalent. Because $\mech_2$ holds certain properties that make later analysis easier, we prefer $\mech_2$ to $\mech_1$. We call $\mech_2$ as the \textbf{standard form} of $\mech_1$, where the query matrix has linearly independent rows and the covariance matrix is an identity matrix. From now on we assume every mechanism is in its standard form for simplicity.
---------



\begin{example}
\label{example:candidate}
Under the same setting in example \ref{example:sumquery}, let's look at a mechanism $\mech_c(x) = \bmat_c x + N(0, \covar_c)$, where $\bmat_c = [1~1~1~1]$, $\covar_c = 5\sigma^2$. The privacy cost matrix of $\mech_c$ is $\Delta_{\mech_c} = \frac{1}{5\sigma^2} \vec{1}^T \vec{1}$, here $\vec{1} = [1~1~1~1]$. Recall that the privacy cost matrix of $\commech$ is $\Delta_{\commech} = \frac{1}{4\sigma^2} \vec{1}^T \vec{1}$, so $\Delta_{\mech_c} \prec \Delta_{\commech} \preceq \Delta_{\mech_1} $, $\Delta_{\mech_c} \prec \Delta_{\commech} \preceq \Delta_{\mech_2} $, which means $\mech_c$ is also a common candidate of $\mech_1$ and $\mech_2$. 
\end{example}

The only difference between $\mech_c$ and $\commech$ is that $\mech_c$ adds more noise to the query answers. Both $\mech_c$ and $\commech$ are common candidates of $\mech_1$ and $\mech_2$, but $\commech$ is more accurate and contains more information of the original mechanisms. Therefore, given many common candidates, it's necessary to find mechanisms that contain most shared information, defined as the (maximally) common mechanism.

\begin{definition}\label{def:maximal}
We say $\commech$ is a \emph{(maximally) common mechanism} to $\mech_a$ and $\mech_b$ if (1) it is a common candidate to $\mech_a$ and $\mech_b$ and (2) if it is not missing information; we formalize this as follows: if there exists an $\mech_c$ that is common to $\mech_a$ and $\mech_b$ and if $\commech$ is answerable from $\mech_c$, then $\mech_c$ is answerable from $\commech$.
\end{definition}
 
By definition \ref{def:maximal}, $\mech_c$ in the example \ref{example:candidate} is not a common mechanism because $\mech_c$ is answerable from $\commech$ but $\commech$ is not answerable from $\mech_c$. In the following subsection, we will focus on finding a common mechanism of two mechanisms.

------------

The proof is based on posts : \href{https://math.stackexchange.com/questions/767882/linear-algebra-vector-space-how-to-find-intersection-of-two-subspaces}{\color{green}{this post}}.

Let $\vec{z}$ be a vector that lies in intersection of two sub-spaces spanned by the rows of $\bmat_a$ and $\bmat_b$. Since $\vec{z}$ is on both sub-spaces, projecting it onto each subspace doesn't change the vector.

Therefore, $\vec{z} = \mat{P}_a \vec{z}$ and $ \vec{z} = \mat{P}_b \vec{z}$.

Substituting one in the other gives $\vec{z}= \mat{P}_a \mat{P}_b \vec{z}$ therefore, $\vec{0}=(\mat{P}_a \mat{P}_b - \mat{I})\vec{z}$.

It means that z is in the null space of $\mat{M} = (\mat{P}_a \mat{P}_b - \mat{I})$. Perform the eigenvalue decomposition on $\mat{M}$ and select the eigenvectors corresponding to zero and that forms an orthogonal basis for the intersection of given sub-spaces.


==> extraexperiments.tex <==








\section{Extra Experiment}

\subsection{Compare 2-way marginals with identity queries}
Here are two mechanisms,
\begin{itemize}
    \item $\mech_1$: $\bmat_1$ is the 2-way marginals, $\covar_1 = 21*\sigma^2 \mat{I}$.
    \item $\mech_2$: $\bmat_2 = \mat{I}$, $\covar_2 = \sigma^2 \mat{I}$.
\end{itemize}
$\bmat_1^T \covar_1^{-1} \bmat_1 = \bmat_2^T \covar_2^{-1} \bmat_2$, so two mechanisms have the same privacy cost $\frac{1}{\sigma^2}$.




\begin{table}[H]
\caption{Compare 2-way marginals with identity queries on HispRace dataset. Experiment with different $\sigma$ when $(x,y)=(0.3, 3)$. }
\centering
 \begin{tabular}{| c | c | c | c | c | }
 \hline
 $\sigma$ & $\rho$ &  \asfname & \ascname  & \algoname   \\ [0.5ex]   
 \hline
 0.1 & 50  & 51.73 & 48.27 & 97.43 \\
   \hline
 0.2 & 12.5    & 63.67 & 36.33 & 96.20 \\
   \hline
    0.3 & 5.56    &  71.88 &  28.12 & 95.50 \\
    \hline
    0.4 & 3.125    & 74.77 &25.23  & 96.05 \\
    \hline
 0.5 & 2   &79.05  & 20.95 & 96.17 \\
   \hline
 $\frac{1}{\sqrt{2}}$ & 1   & 83.45 & 16.55 & 96.67 \\
   \hline
 1 & 0.5  & 88.06 & 11.94 & 97.16 \\
   \hline
 2 & 0.125   & 94.64 & 5.36 & 98.31 \\
   \hline
 4 & 0.031    & 97.99 & 2.01 & 99.26 \\
 \hline
\end{tabular}
\end{table}


\begin{table}[H]
\caption{Compare 2-way marginals with identity queries on HipRace dataset. Experiment with different $y$ when $x=0.3, \sigma=0.5$. }
\centering
 \begin{tabular}{| c | c | c | c |  }
 \hline 
 $y$ &  \asfname & \ascname  & \algoname   \\ [0.5ex]   
  \hline
 1  & 58.30 & 41.70 & 65.88 \\
 \hline
 2  & 71.88 & 28.12 & 89.40 \\
 \hline
 3  & 79.05 & 20.95 & 96.17 \\
 \hline
  4  & 83.45 & 16.55 & 97.54 \\
 \hline
  5  & 86.51 & 13.49 & 98.19 \\
   \hline
  6  & 88.06 & 11.94 & 98.70 \\
 \hline
   8  & 91.36  & 8.64  & 99.18  \\
 \hline
   10  & 93.44  & 6.56  & 99.44  \\
 \hline
   12  &  94.64 & 5.36  & 99.62  \\
 \hline
\end{tabular}
\end{table}

\begin{table}[H]
\caption{Compare 2-way marginals with identity queries on HispRace dataset. Experiment with different $x$ when $y=3, \sigma=0.5$.}
\centering
 \begin{tabular}{| c | c | c | c |  }
 \hline
 $x$ &  \asfname & \ascname  & \algoname   \\ [0.5ex]   
 \hline
 0.2   & 29.53 & 70.46 & 95.57 \\
 \hline
 0.3  & 79.05 & 20.95 & 96.17 \\
 \hline
  0.4  & 88.94 &11.06 & 97.61 \\
 \hline
  0.5  & 94.6 & 5.39 & 98.81 \\
 \hline
  0.6 & 98.29 & 1.71 & 99.52 \\
 \hline
  0.7 & 99.72 & 0.28 & 99.87 \\
 \hline
  0.8 & 99.97 & 0.03 & 99.98 \\
 \hline
\end{tabular}
\end{table}


\subsection{Age Gender}





\begin{table}
\parbox{.49\linewidth}{
\centering
  \begin{tabular}{| c| c | c | c | }
 \hline
 \multicolumn{4}{|c|}{\textbf{2-way vs. Identity}}\\
 \multicolumn{1}{|c}{$\rho$} &  \multicolumn{1}{c}{\asfname} & \multicolumn{1}{c}{\ascname}  & \multicolumn{1}{c|}{Acc}  \\ [0.5ex] 
 \hline
 2   &79.05  & 20.95 & 96.17 \\
   \hline
  1   & 83.45 & 16.55 & 96.67 \\
   \hline
  $1/2$  & 88.06 & 11.94 & 97.16 \\
   \hline
 $1/8$   & 94.64 & 5.36 & 98.31 \\
   \hline
  $1/32$     & 97.99 & 2.01 & 99.26 \\
  \hline
     \multicolumn{4}{|c|}{\textbf{$\%$PLB Saved}: \textcolor{red}{$22.66\%$}}\\\hline
\end{tabular}
}
\caption{Experiments on \textbf{HispRace} dataset as zCDP privacy budget $\rho$ varies. The SNR parameters are  $(x,y)=(0.3, 3)$.}
\end{table}

\begin{table}
\parbox{.49\linewidth}{
\centering
 \begin{tabular}{| c | c | c | c |  }
 \hline 
  \multicolumn{4}{|c|}{\textbf{2-way vs. Identity}}\\
 \multicolumn{1}{|c}{$x$} &  \multicolumn{1}{c}{\asfname} & \multicolumn{1}{c}{\ascname}  & \multicolumn{1}{c|}{Acc}  \\ [0.5ex] 
 \hline
 0.2   & 29.53 & 70.46 & 95.57 \\
 \hline
 0.3  & 79.05 & 20.95 & 96.17 \\
 \hline
  0.4  & 88.94 &11.06 & 97.61 \\
 \hline
  0.5  & 94.6 & 5.39 & 98.81 \\
 \hline
  0.6 & 98.29 & 1.71 & 99.52 \\
 \hline
      \multicolumn{4}{|c|}{\textbf{$\%$PLB Saved}: \textcolor{red}{$50.5\%$}}\\\hline
\end{tabular}
}
\hfill
\parbox{.49\linewidth}{
\begin{tabular}{| c | c | c | c |  }
\hline
 \multicolumn{4}{|c|}{\textbf{2-way vs. Identity}}\\
 \multicolumn{1}{|c}{$y$} &  \multicolumn{1}{c}{\asfname} & \multicolumn{1}{c}{\ascname}  & \multicolumn{1}{c|}{Acc}  \\ [0.5ex] 
 \hline
 3  & 79.05 & 20.95 & 96.17 \\
 \hline
  4  & 83.45 & 16.55 & 97.54 \\
 \hline
  5  & 86.51 & 13.49 & 98.19 \\
   \hline
  6  & 88.06 & 11.94 & 98.70 \\
 \hline
   8  & 91.36  & 8.64  & 99.18  \\
 \hline
      \multicolumn{4}{|c|}{\textbf{$\%$PLB Saved}: \textcolor{red}{$22.66\%$}}\\\hline
\end{tabular}
}
\caption{Experiment on \textbf{HispRace} dataset for zCDP parameter $\rho=2$. Left: SNR parameters $(x, 3)$ as $x$ varies. Right: SNR parameters $(0.3, y)$ as $y$ varies.}
\end{table}





\begin{table}[H]
\caption{Compare 4 mechanisms on AgeGender dataset. Experiemtn with different $y$ when $x=0.5, \rho=\frac{1}{128}$.}
\centering
 \begin{tabular}{| c | c | c | c | c | c| c |  }
 \hline
 $y$ &  $\%\mech_1$ & $\%\mech_2$ & $\%\mech_3$ &$\%\mech_4$  & Acc  &\makecell{\textbf{\% PLB} \\ \textbf{saved}} \\ [0.5ex] 
  \hline
 2  &  0.27  &   0.42 & 0.41  & 98.89  & 99.61  &  49.76\\
   \hline
  7   &  0.36  &  0.85  &  4.55 & 94.23  & 98.80  &   49.61\\
 \hline
   12  &  0.41  & 1.90   &  19.78 &  77.92    & 97.23  &  49.33\\
 \hline
 17 &  0.46  &  5.07    & 39.37  &  55.09 & 96.19  & 48.51  \\
 \hline
22    &  0.52  &  10.44  & 55.44  & 33.60  &  96.24 &  47.14 \\
 \hline
    27    & 0.58   &  17.66  &  63.70 & 18.06  &  96.76 & 45.31 \\
 \hline
\end{tabular}
\end{table}

\begin{table}[H]
\caption{Compare 4 mechanisms on AgeGender dataset. Experiment with different $x$ when $y=20, \rho=\frac{1}{128}$.}
\centering
 \begin{tabular}{| c | c | c | c | c | c| c| }
 \hline
 $x$ &  $\%\mech_1$ & $\%\mech_2$ & $\%\mech_3$ &$\%\mech_4$  & Acc  &\makecell{\textbf{\% PLB} \\ \textbf{saved}} \\ [0.5ex] 
  \hline
 0.2  &0.50  &2.55  &27.86 &69.09 &97.43  &  49.12\\
   \hline
  0.3  &0.50  &6.01  &33.76 &59.72 &96.79  &  48.25\\
 \hline
 0.4  & 0.50  & 8.08  & 42.02 &49.40 &96.27 &  47.74\\
 \hline
  0.5  & 0.50 &8.08  &49.95 &41.47 &96.09 & 47.74\\
 \hline
  0.6  & 0.50 & 12.69 & 60.45 & 26.36 & 95.88  &  46.59\\
 \hline
  0.7  & 0.50 & 15.77  & 72.06 & 11.67 & 96.25  &  45.82\\
 \hline
  0.8  & 0.50 & 39.84 & 56.59 & 3.06 & 95.32  & 39.80 \\
 \hline
\end{tabular}
\end{table}

\begin{table}[H]
\caption{Thresholds on AgeGender dataset. Experiment with different $\rho$ when $(x,y)=(0.5, 20)$.}
\centering
 \begin{tabular}{| c | c | c | c| c| c|
 }
 \hline
 $\rho$  & LR0 & LR1 & LR2   & LR3  & CM \\ [0.5ex]
  \hline
 $\frac{1}{8}$ & 97.71  & 97.71 & 97.68 & 97.63 & 99.80 \\
   \hline
 $\frac{1}{32}$ & 94.59 & 94.50 & 94.16 & 91.70  & 98.74 \\
 \hline
  $\frac{1}{72}$ & 89.03  & 88.91  & 88.06 &  83.17 & 97.32 \\
 \hline
 $\frac{1}{128}$ & 87.02 & 86.86  & 85.60 &  76.70 & 96.09 \\
 \hline
  $\frac{1}{200}$ & 87.57  & 87.18  & 85.02 &  73.59  & 95.88 \\
 \hline
  $\frac{1}{288}$ & 88.81  & 88.30 & 85.17 & 71.63  &95.75 \\
 \hline
\end{tabular}
\end{table}



\begin{table}[H]
\caption{Thresholds on AgeGender dataset. Experiment with different $y$ when $x=0.5,\rho=\frac{1}{128}$.}
\centering
 \begin{tabular}{| c | c |  c | c| c| c|}
 \hline
 $y$  & LR0 & LR1 & LR2   & LR3  & CM \\ [0.5ex]
  \hline
 2  &  99.17 &  99.07  & 99.03   & 98.67  & 99.61\\
   \hline
 7   & 96.17  & 96.17 & 95.88  &  93.32 & 98.80 \\
 \hline
  12    & 92.23  &  91.98 & 90.64    & 84.62  & 97.23 \\
 \hline
 17 &  86.51  & 86.36  & 85.10  & 78.41  &  96.19\\
 \hline
  22   &  87.23 & 87.05  & 85.47   & 76.46 &  96.24\\
 \hline
  27   & 87.90 &  87.67 & 86.23  & 77.54  &  96.76\\
 \hline
\end{tabular}
\end{table}

\begin{table}[H]
\caption{Compare 4 mechanisms on AgeGender dataset. Experiment with different $x$ when $y=20, \rho=\frac{1}{128}$.}
\centering
 \begin{tabular}{| c  | c| c | c| c| c|}
 \hline
 $x$  & LR0 & LR1 & LR2   & LR3  & CM \\ [0.5ex]
 \hline
 0.2    & 92.83   & 92.52 & 90.69 &  80.18 & 97.43\\
   \hline
  0.3    &  89.37  & 89.23 & 87.66 & 78.14  &96.79 \\
 \hline
 0.4    &  88.26   & 88.09 & 86.37 &   76.43 & 96.27\\
 \hline
  0.5    & 87.02 & 86.86  &85.60  &  76.70 & 96.09 \\
 \hline
  0.6    &  86.10 & 85.82 & 84.41 & 75.66  &95.88\\
 \hline
  0.7    & 86.11   &85.85  & 84.73 &  77.93 &96.25\\
 \hline
  0.8    & 73.20  & 73.19 & 72.74 & 69.83  &95.32\\
 \hline
\end{tabular}
\end{table}



\begin{figure}[H]
\caption{Thresholds on AgeGender dataset. Experiment with different $y$ when $x=0.5, \rho=1/128$.}
    \centering
    \includegraphics[width=0.5\textwidth,trim=0.4cm 0.6cm 0cm 0cm]{figs/Table11.pdf}
    \label{fig:agegender-y}
\end{figure}





\begin{figure}[H]
\caption{Compare 4 mechanisms on AgeGender dataset. Experiment with different $x$ when $y=20, \rho=1/128$.}
    \centering
    \includegraphics[width=0.5\textwidth,trim=0.4cm 0.6cm 0cm 0cm]{figs/Table12.pdf}
    \label{fig:agegender-x}
\end{figure}


